Lip-Listening: Mixing Senses to Understand Lips using Cross Modality Knowledge Distillation for Word-Based Models

In this work, we propose a technique to transfer speech recognition capabilities from audio speech recognition systems to visual speech recognizers, where our goal is to utilize audio data during lipreading model training. Impressive progress in the domain of speech recognition has been exhibited by audio and audio-visual systems. Nevertheless, there is still much to be explored with regards to visual speech recognition systems due to the visual ambiguity of some phonemes. To this end, the development of visual speech recognition models is crucial given the instability of audio models. The main contributions of this work are i) building on recent state-of-the-art word-based lipreading models by integrating sequence-level and frame-level Knowledge Distillation (KD) to their systems; ii) leveraging audio data during training visual models, a feat which has not been utilized in prior word-based work; iii) proposing the Gaussian-shaped averaging in frame-level KD, as an efficient technique that aids the model in distilling knowledge at the sequence model encoder. This work proposes a novel and competitive architecture for lip-reading, as we demonstrate a noticeable improvement in performance, setting a new benchmark equals to 88.64% on the LRW dataset.

==> references.tex <==
\begin{thebibliography}{99}

\bibitem{intro2}
Adriana Fernandez-Lopez, and Federico M.Sukno. "Survery on Automatic Lip-Reading in the Era of Deep Learning," in \textit{Image and Vision Computing}, Vol. 78, pp. 53-72, Oct. 2018.

\bibitem{c12}
Abderrahim Mesbah, Aissam Berrahou, Hicham Hammouchi, Hassan Berbia, Hassan Qjidaa, and Mohamed Daoudi. “Lip Reading with  Hahn Convolutional  Neural Networks.” in \textit{Image and Vision Computing}, 2019. 

\bibitem{c13}
Amirsina Torfi, Seyed Mehdi Iranmanesh, Nasser M. Nasrabadi, and Jeremy Dawson, "3D Convolutional Neural Networks for Cross Audio-Visual Matching Recognition," in \textit{IEEE Access}, vol. 5, pp. 22081-22091, 2017, doi: 10.1109/ACCESS.2017.2761539.

\bibitem{c4} 
Brais Martinez, Pingchuan Ma, Stavros Petridis, and Maja Pantic, “Lipreading Using Temporal Convolutional Networks,” in \textit{ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}. IEEE, 2020, pp. 6319–6323.

\bibitem{paper2} 
Bo Xu, Cheng Lu, Yandong Guo, and Jacob Wang, "Discriminative Multi-modality Speech Recognition," in \textit{2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, Seattle, WA, USA, 2020, pp. 14433-14442.

\bibitem{deepspeech2} Dario Amodei, Rishita Anubhai, Eric Battenberg, Carl Case, Jared Casper, Bryan Catanzaro, Jingdong Chen et al., “Deep speech 2: End-to-end Speech Recognition in English and Mandarin,” in \textit{International conference on machine learning},2016, pp. 173–182. https://arxiv.org/pdf/1512.02595.pdf 

\bibitem{withoutpain} 
Dalu Feng, Shuang Yang, Shiguang Shan, and Xilin Chen, “Learn an Effective Lip Reading Model Without Pains,” 2020, https://arxiv.org/pdf/2011.07557v1.pdf  

\bibitem{mg}
Chenhao Wang, “Multi-grained spatio-temporal modeling
for lip-reading,” in \textit{The 30th British Machine Vision Conference(2019)}, 2019.

\bibitem{intro1} 
DouglasO’Shaughnessy, "Invited paper: Automatic speech recognition: History, methods and challenges," in \textit{Pattern Recognition},Vol.41, pp.2965-2979, Oct. 2008.

\bibitem{c10}
Joon Son Chung, Andrew Senior, Oriol Vinyals, and Andrew Zisserman. "Lip reading sentences in the Wild," in \textit{arXiv preprint} arXiv:1611.05358, 2, 2016.

\bibitem{c17}
Joon Son Chung, and Andrew Zisserman, “Lip reading in profile,” 2017

\bibitem{df}
Jingyun Xiao, Shuang Yang, Yuanhang Zhang, Shiguang Shan, and Xilin Chen, “Deformation flow based two-stream network
for lip reading,” in \textit{the 15th IEEE International Conference on Automatic Face and Ges-ture Recognition (FG 2020)}, 2020.

\bibitem{c11}
Kuniaki Noda, Yuki Yamaguchi, Kazuhiro Nakadai, Hiroshi G. Okuno, Tetsuya Ogata. "Lipreading Using  Convolutional  Neural  Network," in \textit{15th  Annual  Conference  of  the  International  Speech Communication Association}. 2014. 


%CONTINUE HERE
\bibitem{c2} 
K R Prajwal, Rudrabha Mukhopadhyay, Vinay Namboodiri, and C V Jawahar, "Learning Individual Speaking Styles for Accurate Lip to Speech Synthesis," in \textit{2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, Seattle, WA, USA, 2020, pp. 13793-13802.

\bibitem{localization2} 
Markus Mathias, Rodrigo Benenson, Marco Pedersoli. and Luc Van Gool, "Face Detection without Bells and Whistles," in \textit{European Conference on Computer Vision 2014 (ECCV).} Lecture Notes in Computer Science, Vol 8692, pp. 720-735, 2014.  

\bibitem{pg} 
Mingshuang Luo, Shuang Yang, Shiguang Shan, and Xilin
Chen, “Pseudo-convolutional policy gradient for sequence-tosequence lip-reading,” in \textit{the 15th IEEE International Conference on Automatic Face and Ges-ture Recognition (FG 2020)}, 2020.

\bibitem{msd}
Pingchuan Ma, Brais Martinez, Stavros Petridis, and Maja Pantic, “Towards practical lipreading with distilled and efficient models,” in \textit{ICASSP 2020-2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 2020.

\bibitem{attention}
 Shivansh Rao, Tanzila Rahman, Mrigank Rochan and Yang Wang, “Video-based Person Re-identification Using Spatial-Temporal Attention Networks,” 2018.
 
\bibitem{localization1} 
Stefanos Zafeiriou, Cha Zhang, and Zhengyou Zhang,"A Survey on Face Detection in the Wild: Past, Present, and future," in \textit{Computer Vision and Image Understanding}, Vol. 138, pp. 1-24, Sept. 2015. 

\bibitem{c16}
Shuang Yang, Yuanhang Zhang, Dalu Feng, Mingmin Yang, Chenhao Wang, Jingyun Xiao, Keyu Long, Shiguang Shan, and Xilin Chen, “Lrw-1000: A naturally-distributed largescale benchmark for lip reading in the wild,” in \textit{2019 14th IEEE International Conference on Automatic Face \& Gesture Recognition (FG 2019)}. IEEE, 2019, pp. 1–8.

\bibitem{c6} 
Triantafyllos Afouras, Joon Son Chung, Andrew Senior, Oriol Vinyals, and Andrew Zisserman, "Deep Audio-Visual Speech Recognition," in \textit{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2019.

\bibitem{c1} 
Triantafyllos Afouras, Joon Son Chung, and Andrew Zisserman. "Deep lip Reading: A Comparison of Models and an Online Application," in \textit{INTERSPEECH}, 2018.

\bibitem{c8}
Triantafyllos Afouras, Joon Son Chung, and Andrew Zisserman, "ASR is All You Need: Cross-Modal Distillation for Lip Reading," in \textit{ICASSP 2020 - 2020 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, Barcelona, Spain, 2020, pp. 2143-2147, doi: 10.1109/ICASSP40776.2020.9054253.

\bibitem{mi} 
Xing Zhao, Shuang Yang, Shiguang Shan, and Xilin Chen,
“Mutual information maximization for effective lip reading,” in \textit{the 15th IEEE International Conference on Automatic Face and Gesture Recognition (FG 2020)}, 2020.

\bibitem{ts} 
Xinshuo Weng and Kris Kitani, “Learning spatio-temporal features with two-stream deep 3d cnns for lipreading,” in \textit{The 30th British Machine Vision Conference(2019)}, 2019

\bibitem{c14}
Ya Zhao, Rui Xu, Xinchao Wang, Peng Hou, Haihong Tang, Mingli Song. "Hearing Lips: Improving Lip Reading by Distilling Speech Recognizers," in
\textit{arXiv preprint arXiv:1911.11502}, 2019.

\bibitem{c5} 
Yuanhang Zhang, Shuang Yang, Jingyun Xiao, Shiguang Shan, Xilin Chen. "Can We Read Speech Beyond the Lips? Rethinking RoI Selection for Deep Visual Speech Recognition," in \textit{CoRR}, abs/2003.03206, 2020.

\bibitem{c9}
Yuanyao Lu, and Hongbo Li. “Automatic Lip-Reading System Based on Deep Convolutional Neural Network and Attention-Based Long Short-Term Memory,”  in \textit{Applied Sciences}, vol. 9, no. 8,  pp.  1599, 2019.

\end{thebibliography}
